Advertising Media and Target Audience Optimization via High-dimensional Bandits

We present a data-driven algorithm that advertisers can use to automate their digital ad-campaigns at online publishers. The algorithm enables the advertiser to search across available target audiences and ad-media to find the best possible combination for its campaign via online experimentation. The problem of finding the best audience-ad combination is complicated by a number of distinctive challenges, including (a) a need for active exploration to resolve prior uncertainty and to speed the search for profitable combinations, (b) many combinations to choose from, giving rise to high-dimensional search formulations, and (c) very low success probabilities, typically just a fraction of one percent. Our algorithm (designated LRDL, an acronym for Logistic Regression with Debiased Lasso) addresses these challenges by combining four elements: a multiarmed bandit framework for active exploration; a Lasso penalty function to handle high dimensionality; an inbuilt debiasing kernel that handles the regularization bias induced by the Lasso; and a semi-parametric regression model for outcomes that promotes cross-learning across arms. The algorithm is implemented as a Thompson Sampler, and to the best of our knowledge, it is the first that can practically address all of the challenges above. Simulations with real and synthetic data show the method is effective and document its superior performance against several benchmarks from the recent high-dimensional bandit literature.

==> secs/old/old_intro.tex <==
\section{Introduction}
% \comm{(HN:Not sure we need to cite this price water house report here. I think at a very high level the important things to bring out in the first para is that targeting at a very fine level is a dominant feature of internet online advertising ; that many possible types of media can be used to Target users. And that the proliferation of options generates lots of uncertainty for advertisers, leading to the need for automation and experimentation to resolve the uncertainty. If we add the point that experimentation in online settings is much more feasible than experimentation in offline settings, that sets up the stage for combining automation with experimentation for addressing these kinds of problems. This is the scope of our paper.)}\\
% According to the PwC Internet Advertising Revenue report,\footnote{See \href{https://s3.amazonaws.com/media.mediapost.com/uploads/InternetAdvertisingRevenueReportApril2021.pdf}{https://s3.amazonaws.com/media.mediapost.com/uploads/InternetAdvertisingRevenueReportApril2021.pdf}.} the U.S. online advertising industry experienced a 30\% growth in total revenue from 2018 to 2020, with display advertising contributing about one-third of the total. A major driver of the industry’s rapid growth is the development of technology that allows advertisers to provide customized ads (called “creatives” in this paper) for different audience segments, allowing precise, real-time targeting of potential customers.

% % cf. \cite{braun2013online}.

% \comm{(Alternative first paragraph) (WB: do you think it's helpful to include some number to highlight the importance of this industry?) With competition coming from all angles and pervasive consumer ``ad blindness,'' advertisers must find ways to reach finely defined audiences with the right ads to make a successful online ad campaign. More than ever, targeting at a very fine level is a dominant feature of internet online advertising, and many possible types of media can be used to create ads. The proliferation of the options generates lots of uncertainty for advertisers, leading to the need for automation and experimentation to resolve the uncertainty.}


The U.S. online advertising industry has grown rapidly in recent years,  and a major driver of that growth is the development of customized ads (called ``creatives'' in this paper) for different audience segments. As the industry progresses from standard demographic targeting criteria (for example, age, gender and geography) to contextual criteria (for example, what webpages a user is browsing) to behavioral criteria (past actions), the number of possible target audience segments grows rapidly. Moreover, there are often many potential creatives, using a variety of different media, for a given target audience. The combination of these factors leads to \textit{high-dimensional} matching problems, by which we mean that the number of potential audience-ad combinations is large relative to the amount of experimentation that an advertiser can conduct. Proliferation of targeting options increases advertiser uncertainty, and consequently increases demand for automated experimentation to resolve that uncertainty. Our paper is focused on methods for managing or guiding such experimentation, in order to deliver the most effective creatives to potential customers.

However, there are several obstacles to successful experimentations. Success rates are low for online ads, with an average click-through rate (CTR) below 0.5\% according to a recent report.  Thus, in an ad campaign where 1 million impressions are allocated evenly among 1000 combinations of audience and ad, each combination expects to receive fewer than five clicks (positive responses). Therefore, getting accurate CTR estimates using traditional testing methods, where experiments are evenly divided among competing alternatives, may be prohibitively expensive in high-dimensional settings. This motivates two central features of the methods discussed in this paper: adaptive sampling and cross learning. In our context, “adaptive sampling” means that as experimentation progresses, sampling is biased toward alternatives that have shown greater promise. “Cross learning” means that results from a single audience-ad pair are used, in combination with a statistical model, to make inferences about the effectiveness of other pairs as well. 

Another important consideration in an online setting is latency, because a matching result usually has to be out within 100 ms, cf. \cite{wang2016display}. The amount of computation required for statistical analysis will increase dramatically as problem size (that is, the number of audience-ad combinations considered) increases, so it is important to streamline computations. 

In this paper, we consider two models of sequential decision-making for online advertising. In the first of them, called the \textit{single-stage model}, decisions are made by the advertiser, or rather by an algorithm that the advertiser provides. For each trial $t = 1, 2, \dots , T,$ the advertiser’s algorithm chooses a \textit{target audience} (TA) for which to purchase an impression, and simultaneously chooses a \textit{creative} (CA) to display for a user chosen at random from that audience segment. The algorithm then observes a binary outcome in the form of click or no-click. Building on previous work in the field, the advertiser’s problem is cast as a multi-armed bandit, and more specifically as a \textit{Bernoulli bandit}, with (TA, CA) combinations playing the role of ``arms''. The advertiser aims to make TA and CA choices to maximize the expected click-through rate achieved in a total of $T$ trials.

In our second, two-stage model, it is the platform that conducts experiments, using an automated algorithm to optimize an ad campaign on behalf of the advertiser. Compared to the advertiser, the platform is likely to have more information that it privately observes about arriving impressions, and it can use that finer information in choosing the CA presented to a user, instead of basing the choice on just the broadly defined TA from which the user is drawn. Therefore, in our second model the problem is treated as a contextual bandit. We will compare the click-through rates achieved in these two different learning regimes, characterizing the difference as the benefit that an advertiser realizes by having a platform conduct experiments on its behalf.

% \comm{
% As the industry progresses from standard demographic criteria (observed demographics like age, gender, and geography) to contextual targeting criteria (what webpages a user is browsing), to behavioral criteria (past actions), ads can be targeted more finely, which makes the number of possible targeting segments large. Moreover, each target segment could respond differently to different kinds of media, leading to the proliferation of creatives. As a result, it is increasingly common to see an advertiser testing tens or even hundreds of creatives and target segments in an ad campaign. The combination of these factors leads to \textit{high-dimensional} matching problems, by which we mean that the number of potential audience-ad combinations is large relative to the amount of experimentation that an advertiser can conduct. }

% \comm{(old version)}\cite{elgammal2017can} describe new technologies for generating differentiated creatives in an automated fashion, leading to large arrays of potential creatives for a given target audience. As a result, it is increasingly common to see an advertiser testing tens or even hundreds of creatives in an ad campaign. In addition, ads can be targeted more finely as the industry progresses from standard demographic criteria (like age, gender, and geography) to contextual targeting criteria (for example, what webpage a user is browsing, or behavioral information about the user). The combination of these factors leads to \textit{high-dimensional} matching problems, by which we mean that the number of potential audience-ad combinations is large relative to the amount of experimentation that an advertiser can conduct. 

% % As noted by \cite{geng2020comparison} and others, high-dimensional matching problems present obvious challenges for marketers. Traditional testing methods typically require many user samples, which can be prohibitively expensive in high-dimensional settings, and the number of online computations required for statistical analysis may increase dramatically as the problem dimension increases. Furthermore, in an online setting,  latency  becomes an important consideration, since a matching result usually has to be out within 100 ms, cf. \cite{wang2016display}. Thus, streamlining computations for a learning algorithm is important.  

As noted by \cite{geng2020comparison} and others, high-dimensional matching problems present obvious challenges for marketers. Traditional testing methods typically require many user samples, which can be prohibitively expensive in high-dimensional settings. Furthermore,  in an online setting, latency becomes an important consideration, because a matching result usually has to be out within 100 ms, cf. \cite{wang2016display}. The amount of computation required for statistical analysis will increase dramatically as the problem size (the number of possible combinations) increases, so it is important to streamline the computations for a learning algorithm.

Moreover, success rates for online advertising are low, with an average value below 0.5\% according to a recent report.\footnote{See \href{https://www.wordstream.com/blog/ws/2016/02/29/google-adwords-industry-benchmarks}{https://www.wordstream.com/blog/ws/2016/02/29/google-adwords-industry-benchmarks}} Thus, in an ad campaign where 1 million impressions are allocated evenly among 1000 combinations of audience and ad, each combination expects to receive only about five clicks (positive responses). This makes click-through rate (CTR) estimation for any given combination difficult. In such an environment, a crucial consideration is \textit{cross-learning}, by which we mean the use of results for many or all audience-and-ad combinations in estimating the CTR for any one combination. To express that same point in general statistical language, the use of \textit{indirect evidence} can be crucial when response rates are low. \comm{(HN:The issue of cross learning seems to be a key contribution of our paper and it seems to me that it deserves to be emphasized more in the introduction)  }
% Despite the remarkable line of work we just mentioned, as well as the recent progress in high-dimensional bandits (\cite{wang2018minimax}, \cite{kim2019doubly}, \cite{bastani2020online}, \cite{oh2020sparsity}, \cite{li2021simple}, \cite{fan2021sample}), this remains an open problem.

In this paper, we consider \comm{models of sequential decision-making in an online advertising platform, where the experiment is either conducted by an advertiser or by a platform, in which trials are indexed by $t = 1, 2, \cdots, T$. In our canonical model, for each trial, the advertiser's algorithm chooses a \textit{target audience} (TA) for which to purchase an impression, and a \textit{creative} (CA) to display for a user chosen at random from that audience segment. The algorithm then observes a binary outcome in the form of click or no-click. Building on previous work in the field, the advertiser's problem is cast as a multi-armed bandit problem, specifically a \textit{Bernoulli bandit}, with (TA, CA) combinations playing the role of ``arms''. The advertiser aims to make TA and CA choices to maximize the expected click-through rate (CTR) achieved in a total of $T$ trials. In our second model, the platform offers automation algorithms that optimize campaigns on behalf of the advertiser. Compared to the advertiser, the platform is likely to have more information that it privately observes about arriving impressions, which allows it to learn a contextual policy for which CA to play for each user from the broadly defined TA. Therefore, in the second model, which features the platform running algorithm and involves the utilization of the side information, the problem is treated as a contextual bandit. We will examine the performance of the algorithm in the context of these two different learning regimes, where the difference captures the benefit to an advertiser by having a platform conduct experiments on her behalf.}

As noted earlier, particular attention is focused here on\textit{ high-dimensional bandit} problems. Despite scattered recent progress cited below, the efficient solution of high-dimensional bandits remains in many respects an open problem.

\noindent\textbf{Related work.} \quad Our paper is  related to the literature from three fields: marketing, operations, and machine learning. For a comprehensive survey of recent progress in display advertising, we refer readers to \cite{choi2020online}.

Our work relates to the \comm{marketing and }operations literature on online advertising, one branch of which looks at how to bid in online auctions, cf.  \cite{chapelle2015offline}, \cite{balseiro2015repeated}, \cite{baardman2019scheduling},  \cite{balseiro2019learning},
\comm{
\cite{waisman2019online},
\cite{tunuguntla2021near}
}
. Another branch of the literature examines how to schedule different ads \citep{turner2012planning,hojjat2017unified}. In addition, there is extensive literature on successful applications of bandits in web content optimization, e.g., \cite{agarwal2009explore}, \cite{li2010contextual}, \cite{chapelle2011empirical}, \cite{agarwal2014taming}, \cite{urban2014morphing}, and \cite{agarwal2016making}. Also notable is the 
comprehensive survey by \cite{wang2016display} of challenges and recent algorithms in real-time bidding (RTB) ecosystems. Our work is most closely related to the substream of this literature that uses bandits for controlled experiments in online platforms. The works closest to ours are \cite{scott2015multi}, \cite{schwartz2017customer}, \cite{ju2019sequential}, and \cite{geng2020comparison}, which propose using bandit experiments to evaluate the effectiveness of different creatives for targeted advertising. 
In contrast to our work, however, \comm{none of the previous papers have shown how to do exploration and exploitation simultaneously over such a large high-dimensional space in the specific context of targeted online advertising.}

% none of the aforementioned works is directly applicable to high-dimensional problems. 

% In our online advertising application domain, the feature spaces are generally high-dimensional, yet frequently only a small subset of features influence the response. It is challenging to identify this small subset of influential features, especially when the data are not as informative due to low CTR. 
Recently, there has been significant interest in contextual bandit problems with high-dimensional feature vectors, cf. \cite{abbasi2012online}, \cite{pmlr-v22-carpentier12}, \cite{gilton2017sparse}, \cite{wang2018minimax}, \cite{kim2019doubly}, \cite{bastani2020online}, \cite{hao2020high}, \cite{oh2020sparsity}, and \cite{li2021simple}. Most studies have focused on linear models, cf. \cite{abbasi2012online}, \cite{gilton2017sparse}, \cite{wang2016display}, \cite{kim2019doubly}, and \cite{bastani2020online}. Only very recently, the work of \cite{oh2020sparsity} expands the model to a generalized linear setting, and further eliminates a critical restriction that was commonly seen in earlier papers, namely, the algorithm needs to know the sparsity index (number of nonzeros in the parameter vector). \cite{oh2020sparsity} study an exploration-free or ``greedy'' method, justified by strong regularity assumptions on the distribution of the user feature vectors. One particular assumption they rely on is \comm{the so-called \textit{relative symmetry condition} which implies} that all intercepts in their high-dimensional linear models are zero. \comm{As nicely articulated by \cite{bastani2021mostly} and \cite{russo2017tutorial}, when there are enough randomness in the context (ensured by the relative symmetry condition), it generates sufficient exploration hence additional active exploration is not necessary. On the other hand, exploration becomes generally necessary when we do not have covariate diversity (e.g., the covariate vector includes the intercept term as in our setting). } \comm{Unfortunately, in our setting with binary covariates and a significant intercept term (the average CTR is low), the relative symmetry condition does not hold and active exploration is needed.}  
\cite{li2021simple} propose a unified framework suitable for high-dimensional bandit problems, including the lasso bandit and matrix bandit. Their analysis of the lasso bandit shares a form similar to that of \cite{oh2020sparsity}, relying on a regularity condition that is hard to meet in our setting. Our real-data experiment (Subsection \ref{subsec:real}) testifies that exploration is important in the low CTR setting. 

Our proposed method, using a Poisson model with debiased lasso estimates (PMDL), modifies the high-dimensional estimator of \cite{javanmard2014confidence} to develop a multi-armed bandit algorithm.
\comm{(HN: explain more about Javanmard 2014 before we get into fan et als paper; Also can we explain what is the implication of the fact that the "standard sparsity assumption on the information matrix is not satisfied in our case; Also, when we say our method is tailored to the challenges encountered in real applications, what are those challenges? Can we explain?)
\cite{javanmard2014confidence} describes a method to remove bias in the lasso estimator and construct confidence regions for linear regressions. The confidence regions provided can be used for active exploration, which is crucial in our setting with binary covariates and a significant intercept term.} This approach is inspired by the working paper of \cite{fan2021sample}, which studies a sampling-based method for high-dimensional \textit{linear contextual bandits}, also using the result of 
% distributional approximations of the Debiased Lasso estimator in 
\cite{javanmard2014confidence}. \comm{We differ from their work mainly in two aspects. First, our method is tailored to the challenges encountered in real applications, e.g., binary response, scarce feedback, as described JD.com in \cite{geng2020comparison}.} Second, they focus on the linear setting, whereas our method addresses a generalized linear model (GLM). The extension from linear to GLM is nontrivial. As noted by \cite{xia2020revisit}, a direct application of \cite{javanmard2014confidence} to a GLM setting may suffer inefficiencies because the standard sparsity assumption (the number of nonzero elements is small) on the information matrix is generally not satisfied, \comm{which makes the resulting confidence regions have a much lower coverage probabilities}. We specifically modify the approach in \cite{javanmard2014confidence} to address this issue.
% our algorithm design reflects the constraints imposed by real-world implementation: computation time, short experiment time, adjustable exploration rate, etc. 

In summary, our paper fills a gap in the literature by addressing these challenges that arise in online advertising: the need for active (and intelligent) exploration in high-dimensional settings, low success probability, and the need for rapid computation.
 
 % \subsection{Paper Overview}
\noindent\textbf{Overview.} \quad Section \ref{sec:problem} contains a precise formulation of the basic problem described above, and Section \ref{sec:method} lays out our proposed solution method. Section \ref{sec:Numerical} presents the results of numerical experiments in which our proposed PMDL method is compared against various alternative approaches for both small and large test problems. We find that the PMDL method is competitive with the best-known alternatives for small problems, and it remains computationally feasible on large problems for which no feasible alternative methods are known. 

In Section \ref{sec:twostage} we extend our analysis of the basic problem to a more complicated setting, \comm{which is motivated by the increasing propensity of tech platforms to offer automation algorithms that optimize campaigns on behalf of their advertisers. In this setting, the platform uses an algorithm to pick from a set of candidate CA's and TAs for the advertiser in each impression opportunity, while learning which CATA combination is best for the advertiser. Compared to the advertiser, the platform is likely to have more information that it privately observes about arriving impressions which allows it to learn a contextual policy for which CA to play for each broadly defined TA.} This is a kind of \textit{contextual bandit problem}, cf. \cite{li2010contextual}. Again, we find that a variant of our PMDL method is computationally feasible for high dimensional problems where no alternative methods are available. The profit increase realized in this more complicated setting, relative to what is achievable by the advertiser in our basic model, can be interpreted as \comm{the benefit realized by outsourcing automation to the platform from the advertiser's perspective.}


%  an advertiser from having its ad-audience experiments conducted by the platform, rather than conducting the experiments itself. 

% in which the advertiser first specifies a target audience (TA) for which an impression is to be purchased, then observes more detailed demographic information about the user actually selected from that TA, and finally chooses a CA for display based on this more detailed information. 


In Section \ref{sec:discussion} we discuss some secondary topics related to our proposed method and its performance in numerical experiments:  the performance gains using adjustable exploration, the performance gains from model refinement, \comm{the essential role of debiasing}, and a method suitable for general success rates. Finally, Section \ref{sec:conclusion} summarizes our paper's contributions and offers a few concluding remarks.



==> secs/old/old_model.tex <==

\section{Single-stage problem}  \label{sec:problem}

\comm{The advertiser can algorithmically choose from a set of target audiences (TAs) $ \KK = \{1, \cdots, K\} $ provided by the platform\footnote{\comm{The platform is motivated to keep the number of TAs available to advertisers manageable, because of the need to operate an impressions market for each TA in the collection. That is, the platform seeks to avoid problems associated with ``thin'' markets. When TAs are defined narrowly, a platform may have difficulty satisfying the demand for impressions, simply because of limited supply. Further, there is a risk that the number of advertisers interested in a narrowly defined TA will be small, leading to weak auction pressure and poor revenue extraction. Also, with a small number of advertisers, the success of such an auction may be overly dependent on the platform’s reserve price, which is difficult to tune given the limited number of transactions occurring for such TAs.}} (e.g., ``San Francisco users'', ``Male users''), and a set of creatives (CAs) $\RR = \{1, \cdots, R\}$ she has available, to run a campaign that optimizes over the best creative-target audience (CA-TA) combinations.}




% The advertiser provides a set of target audiences (TAs) $ \KK = \{1, \cdots, K\} $, which may have overlap (e.g., ``San Francisco users'', ``Male users''), and a set of creatives (CAs) $\RR = \{1, \cdots, R\}$, to design a campaign to find the best creative-target audience (CA-TA) combination. 

At the beginning of each trial $t$, the advertiser submits a CA-TA combination $(r_t, k_t)$ to the platform. The platform randomly chooses one user from that TA and displays the creative $r_t$ to that user. After the creative is displayed, the user's reaction $y_t \in \{0, 1\}$ is observed, with $1$ corresponding to a click and 0 corresponding to a no-click. \comm{For the purpose of this paper, we formulate the problem as one of finding the option with the highest click-through rate, similar to many past papers in the literature, abstracting away from the problem of simultaneously learning an optimal bidding policy. Therefore, the 
 payoff to the advertiser from the ad-impression is}
\[   \pi_{rkt} = y_{rkt}. \]
% The payoff to the advertiser from the ad-impression is
% \[   \pi_{rkt} = \gamma y_{rkt} -  b_{rkt}, \]
% where $\gamma$ is a factor that converts the user's click to monetary units, $y_{rkt} $ is the consumer's response, and $ b_{rkt}$ is the cost of displaying creative $r$ to customer from TA $k$ at time $t$. 
% For the purpose of this paper, we focus on CTR maximization, which is equivalent to the setting where $b_{rkt} = 0 $ and $\gamma = 1$, those factors being known to the advertiser. 
This will allow us to frame the advertiser's problem as a multi-armed bandit (MAB) to maximize CTRs, with the ``arms'' being  CA-TA pairs. 
\footnote{The focus on CTR is particularly relevant for an e-commerce platform such as JD.com\citep{geng2020comparison}: in most cases, the click will directly land the customer on a product page, thereby generating awareness and visibility for the product. Extending the performance criterion to other metrics such as conversion will be valuable, but conversion is rarer, fast-changing, and much harder to track. Further, as noted in \cite{choi2020online}, targeting users based on their conversion probability may not be a good practice, since it suggests serving ads to users who are likely to convert even without ad exposures.}
% ($\gamma$) or revenue will be valuable, although more challenging since conversion is much rarer and harder to track (delayed feedback, etc.) than CTRs. Note that the model, algorithm, and analysis can be directly extended to the case with general $\gamma$ and $b_{rkt}.$ 
Assume the CTR of a user from TA group $k$ after seeing creative $r$ is $p_{rk}$, so that the advertiser's expected reward at time $t$ from choosing the CA-TA combination $(r_t, k_t)$ becomes
  $\pi_t =\EE(y_{rkt}) = p_{r_t k_t}$. The expected reward of the best CA-TA combination is
\eqss{
 \pi^* &= \max_{r,k} ~p_{r k},~\text{and}~ (r^*, k^*) \text{~is the maximizer.}
}

% The DA groups are generated by partitioning all users in $K$ TAs into a set $\JJ = \{1, \cdots, J\}$ of $J$ DAs. For example, if the TAs are $ \{  \text{``San Francisco user''},\text{``Male user''}  \}$, then the DAs are $\{$ ``San Francisco, male user'',``San Francisco, not-male user'', ``not-San Francisco, male user'', ``not-San Francisco, not-male user'' $\}$. Note with $K$ TAs, there may be an exponential amount ( $J \sim 2^K$) of DAs, which results in a high-dimensional learning problem. We denote by $\PP(j|k)$ the proportion of DA $j$ in TA $k$. 

The goal of the advertiser is to maximize her expected total reward  $ \sum_{t=1}^T \pi_{t}$ over the course of $T$ trials. Equivalently, the advertiser is minimizing the pseudo-regret \citep{audibert2009exploration}, which is defined as
\eqs{  \nonumber R_T&=  T\cdot \pi^* -  \sum_{t=1}^T p_{r_t k_t} \\
& \label{eq:regret} 
= \sum_{t=1}^T (  \pi^*   - p_{r_t k_t} )
}
\comm{(HN:Rather than go through this setup and normalize gamma to 1 and bids to 0, is it not simpler to start with the next equation on the next page on pi star directly and simply state that we formulate the problem as one of finding the option with the highest click-through rate, similar to many past papers in the literature, abstracting away from the problem of simultaneously learning an optimal bidding policy. )}

This model deviates from previous work by \cite{geng2020online}, in that we directly address the decision problem confronted by an advertiser, instead of the design of a preliminary experiment conducted by the platform on behalf of the advertiser. A variant of our basic model (Section \ref{sec:twostage}) can be interpreted as the platform's problem, where the experimenter has more information after a user's arrival, and has the flexibility to select a creative based on that additional information.



% \subsection{Three scenarios}

% We consider three distinct formulations that differs in the information provision and process flexibility: 
 
% \begin{itemize}
%     \item Scenario 1 (S1): Advertiser sees only $y_t$ (click or no-click) after each trial.
%     \item Scenario 2 (S2): Advertiser sees $y_t$ and is also told the user's DA information $j_t$ ex-post.
%     \item Scenario 3 (S3): Advertiser has additional flexibility comparing with scenario 2. She sees $y_t$ and is told the user's DA information $j_t$ ex-ante. Thus, the advertiser can select creative $r_t$ contingent on DA information.
% \end{itemize}

% The scenario 1 and scenario 2 has the same control and differ in the information provision and we define their reward difference as the value of information (VOI). The scenario 3 and scenario 2 have the same information and differ in the process flexibility, therefore, we define their reward difference as the value of flexibility (VOF). We will formally define VOI and VOF in section \ref{2sec:method}.

% % Right now every advertiser can do scenario 1 at almost every platform: an advertiser can just go to a platform, specifies a TA group, and provide one creative. S2 & S3 involves more information or flexibility,  which needs the platform to do more. We can easily imagine a time in near future, due to the competitions and the benefits we are about to explain, a platform will be in scenario 2 or scenario 3. In fact, something like S3 is realized in JD platform , and you can sign up for the experiment for free.

% The problem formulation of each scenario is summarized below. It worth noting that due to the added flexibility, the objective value of scenario 3 is larger than the first two, thus the regret measure is also different and actually is usually higher in scenario 3.

% \begin{table}[H]   
%         \centering
%          \begin{adjustwidth}{-1cm}{}
%         \begin{tabular}{|| c|| c |c |c ||}
%          \hline
%           & Scenario 1 &  Scenario 2 &Scenario 3\\ 
%          \hline
%         Information  &   $y_t$ & $y_t, j_t$ (ex-post) & $y_t, j_t$ (ex-ante)\\ [0.5ex] 
%          \hline  
%         Control & $(k_t, r_t)$ &  $(k_t, r_t)$ &  $k_t, f_t: DA \rightarrow CA$  \\ 
%          \hline
%          Objective & $\max \sum_{t=1}^T \sum_j \mathbb{P}(j|k_t)~ p_{r_t j} $ & $ \max \sum_{t=1}^T \sum_j \mathbb{P}(j|k_t)~ p_{r_t j} $ & $  \max \sum_{t=1}^T \sum_j \mathbb{P}(j|k_t)~ p_{f_t(j) j} $
%     \\
%          \hline
%          Regret & $T\cdot \pi^* -\sum_{t=1}^T \sum_j \mathbb{P}(j|k_t)~ p_{r_t j} $& $T\cdot \pi^* -\sum_{t=1}^T \sum_j \mathbb{P}(j|k_t)~ p_{r_t j} $ & $T\cdot \pi^{*'} -\sum_{t=1}^T \sum_j \mathbb{P}(j|k_t)~ p_{f_t(j) j} $\\
%          \hline
%         Effective dim & $R\cdot K$ & $R\cdot J \sim R \cdot 2^K$& $R\cdot J \sim R \cdot 2^K$ \\
%      \hline \hline
%         \end{tabular} 
%     \end{adjustwidth}
%         \linebreak 
%     \caption{Problem formulations for different scenarios.}
%     \label{tb:scenario_objs}
%     \end{table}



==> secs/old/old_pmdl_method.tex <==
\section{Proposed PMDL method}  \label{sec:method}

Our method, Poisson Model with Debiased Lasso (PMDL), is designed to address the challenges described earlier, i.e., active exploration in high-dimensional problems, low CTR, and the need to streamline computation. 
% is designed to address the high-dimensional issue and facilitate cross-learning. 
It consists of three components. The first is a probability model (Subsection \ref{2sec:prob}) that specifies click-through probabilities in terms of more basic parameters. We use a Poisson regression model to accommodate the low CTR, which also reduces the computation time (the time for updating model parameters, e.g., time involved in performing Algorithm \ref{alg_debiasedLasso}). The second component is an estimation method (Subsection \ref{2sec:estimation}), that is, a method for estimating model parameters based on past data as it accumulates. We modify the method from \cite{javanmard2014confidence} to our setting, to perform inference on high-dimensional data. Finally, for treatment selection (that is, choice of an action based on the current parameter estimate), we propose a frequentist version of Thompson sampling, generalized to allow an adjustable degree of emphasis on exploration; this last component of the PMDL method is described in Subsection \ref{2sec:treatment}.

% \begin{enumerate}
%     \item  Probability model (section \ref{2sec:prob}), which specifies click-through probabilities in terms of more basic parameters
%     \item  Estimation method (section \ref{2sec:estimation}): Specifies a method for estimating basic parameters based on past data, as it accumulates 
%     \item Treatment selection (section \ref{2sec:treatment}): Specifies a means of selecting an action for the next stage, based on the estimation result
% \end{enumerate}

\subsection{Hybrid Poisson regression model} \label{2sec:prob}

We assume that the user's feedback $y_{rk}$ is Bernoulli-distributed: $y_{rk} \sim \text{Ber}(p_{rk})$. For modeling of $p_{rk}$, the previous literature primarily fall into two categories: \textit{(i)} $p_{11},\cdots, p_{RK}$ independent with $p_{rk} \sim \text{ Beta} (\alpha_{rk}, \beta_{rk})$, versus \textit{(ii)} logistic regression model, $p_{rk}  = (1+\exp(\theta^\top \phi(r,k)))^{-1}$, where $\phi(r,k)$ is the feature vector to be explained below.

Approach \textit{(i)} is computationally convenient thanks to the self-conjugacy property of the beta distribution, and has been successfully implemented by \cite{geng2020comparison}. However, this means that when we perform updates in the algorithm, the CTR estimate of each CA-TA pair is updated independently. In reality, the chances are that the CA or TA status carries important information, and the CTRs for pairs that share the same CA or TA are correlated. Thus, a method that assumes independence among different pairs may be statistically inefficient. Approach \textit{(ii)} is broadly applicable for a wide range of CTRs. However, it generally needs more computation time than the Poisson model (Subsection \ref{subsec:LMDL}). 

In our regime where the success rate (CTR) is low, a binomial process can be well approximated by a Poisson process \citep{arratia1990poisson}. Motivated by this, we adopt a Poisson regression model for cumulative clicks. 
% To facilitate cross-learning and exploit the low CTR environment, o
Specifically, our proposed PMDL method uses 
\eqs{\label{eq:poisson_model}
p_{rk}  = \exp(c_0 + \alpha_r + \beta_k + \gamma_{rk}),
}
where $c_0, \alpha_r, \beta_k,\gamma_{rk}$ represents the ``baseline effect'', ``CA effect'', ``TA effect'', and the ``additional joint effect'', respectively. All parameters ($c_0, \alpha_r, \beta_k, \gamma_{rk} $) are initially unknown to the advertiser and need to be learned through experimentation. In the standard bandit form, this can be expressed as 
\eqs{p_{rk} = \exp(\theta^\top \phi(r,k)),}
where 
\eqs{  \label{eq:phi}
\phi(r,k) & = \big(1,  \one_{1}(r),\one_{2}(r), \cdots, \one_{R}(r), \one_{1}(k), \one_{2}(k), \cdots, \one_{K}(k), \one_{1,1}(r,k), \cdots, \one_{R,K}(r,k) \big)^\top,\\ \label{eq:coef}
\theta &= \bigl( c_0, \alpha_1, \cdots,  \alpha_R,  \beta_1, \cdots,\beta_K, \gamma_{11},    \cdots \gamma_{RK} \bigr),
}
and $ \one_{x'}(x) = \one(x'=x )$ is the indicator function of $x'=x$. The feature vector $\phi(r,k) $ consists of a 1 for the intercept and indicators for CAs, TAs, and for CA-TA interactions. The unknown parameter vector $\theta$ consists of $c_0,\alpha_r, \beta_{k}$ and $\gamma_{rk}$ values. 

To remove redundant variables in $\theta$ , we impose zero-sum constraints $ \sum_r\alpha_r= \sum_k \beta_k=0$ and $\sum_r \gamma_{rk} = \sum_{k} \gamma_{rk}$ (for all $r$ and $k$). As suggested in Subsection 4.3 of \cite{buhlmann2011statistics}, the parametrization of the feature vector can be simplified by dropping redundant parameters (e.g., dropping $\alpha_R$, $\beta_K,$ and any $\gamma_{rk} $ that has $R$ or $K$ as part of its subscript).\footnote{\comm{This can be automatically implemeted by using the function \pkg{model.matrix} in the \pkg{R} software environment.}}  With this assumption, our PMDL method has $d = (R-1) + (K-1) + (R-1)(K-1)+1 = RK $ parameters to estimate, which equals the total number of unknown CTRs that we are trying to estimate. At the first glance, it may seem that using this probability model does not help us reduce the number of parameters that need to be estimated. Fortunately, under the sparsity assumption that is standard for high-dimensional problems, the inferential approach (debiased Lasso) that we use for PMDL allows us to identify and estimate the actual influential (non-zero) parameters, thereby inducing cross-learning (see Subsection \ref{2sec:estimation}).

The probability model described in this subsection is a special case of the \textit{factorization machine model}, which has been very successful in \comm{estimating CTRs} in various recommendation systems cf. \cite{rendle2010pairwise} and \cite{ menon2011response}.\comm{(HN:also briefly explain what's different here from those applications?) Different from the previous work that focuses on estimation and prediction, we demonstrate the usage of this model in the \textit{learning} setting - when combined with lasso estimation, it encourages cross-learning and helps exploration.}
    
\subsection{Debiased lasso for parameter estimation} \label{2sec:estimation}

The estimation method we use is adapted from \cite{javanmard2014confidence}, which in turn builds on the lasso estimator.
% belongs to the high-dimensional statistics literature. 
% An excellent recent book in this field is \cite{buhlmann2011statistics}. 
The lasso (least absolute shrinkage and selection operator), first proposed in \cite{tibshirani1996regression}, is a popular method for simultaneous estimation and variable selection in high-dimensional models, while retaining computational feasibility for most applications. Unfortunately, this method yields biased estimators, and it is difficult to quantify the uncertainty of estimates and perform statistical inference. Until very recently, there were no principled approaches for obtaining confidence regions for high-dimensional parameters. In 2014, three papers \citep{javanmard2014confidence,van2014asymptotically,zhang2014confidence} proposed related approaches for constructing confidence intervals for lasso estimates by ``debiasing'' the original lasso estimator, i.e., by adding (relatively small) terms to the original lasso estimator to yield an unbiased estimator. They show that this debiased lasso estimator has desirable theoretical properties, retains computational feasibility, and performs well empirically. In this paper, we choose the estimator proposed by \cite{javanmard2014confidence}, both for its computational tractability and because it requires the fewest number of tuning parameters among the three aforementioned estimators.

% \comm{(Shall we keep this paragraph?) Although the debiased lasso estimator's application is straightforward, establishing the regret bound for this problem is highly nontrivial. The bandit policy induces non-i.i.d. samples. 
% % In particular, even the environment is stable and generates i.i.d. samples, the platform will first screen users based on the TA criteria specified by the algorithm. Further, 
% In our setting, the feature vector calculated based on (CA, TA) depends on the action chosen at the beginning of each trial, which is chosen based on the actions and feedbacks from the past. Therefore, the future actions depend on the historical actions, which induce non-i.i.d features. In the low-dimensional setting, a general approach to address the dependency problem is to use the martingales and the method of mixtures (summarized in \cite{lattimore2020bandit}, P. 220). However, this can not be directly applied to the high-dimensional estimator without substantial work. We hope to tackle this problem soon.} 

The debiased lasso estimator builds estimates for $\theta$ (and hence for $p_{rk}$) based on historical data. To start, we express the history in an aggregated form. Let $n_{rk}$ be the number of trials in which the combination $(r, k)$ has been selected, and $s_{rk} $ the number of clicks observed in those trials, up to and including time $t-1.$ At time $ t$, the data available for the algorithm consists of $\cH_t = \{ (n_{rk}, s_{rk}), r  = 1, \cdots , R, k = 1, \cdots, K \}$. 

% Instead of a Bayesian approach that computes the posterior distribution of $p_{rk}$, \


Because \cite{javanmard2014confidence} developed their method for a standard \textit{linear} statistical model, it must be modified for use with our Poisson regression mode, which is an example of a \textit{generalized} linear model (GLM). As \cite{xia2020revisit} have observed, a direct extension of \cite{javanmard2014confidence} to GLM setting may cause bias and an unreliable confidence region, because the key sparsity assumption on the inverse information matrix (the number of nonzeros is small) may not hold \comm{-- in the GLM setting, the inverse information matrix depends on the unknown parameter vector, and with the covariates generally correlated, the off-diagnal terms are non-zero.} Instead, for the computation of the sample covariance matrix, we adopt the approach in \cite{xia2020revisit} where we directly invert the empirical covariance matrix \eqref{eq:dl_cov}. Thanks to the Poisson probability model, the empirical covariance matrix is always invertible. Let $ x_{rk} = \phi(r, k) \in \RR^d$. (Recall that, for each arm or action $(r,k)$ in our model, the corresponding feature vector $\phi(r,k)$ has dimension $d=RK$ after its redundant components are removed.) The debiased lasso estimator $ \hat{\theta}_d$ and its corresponding covariance matrix $\hat{\Sigma}_d$ are computed as follows (Algorithm \ref{alg_debiasedLasso}).



% Notice that 
%  focus on the \textit{linear model}, where they developed theory to approximate the sampling distribution of the $\theta$ estimator. 

% However, a direct extension of their method to the nonlinear setting may suffer inefficiency as . Instead of using their node-wize 

% Their method provide a debiased lasso estimator $ \hat{\theta}_d$ and its corresponding covariance matrix $\hat{\Sigma}_d$ under the linear setting. We adapt their method to GLM, and use 



\begin{algorithm}
\KwIn{c, history  $\cH_t = \{ (n_{rk}, s_{rk}), r  = 1, \cdots , R, k = 1, \cdots, K \}$. \\ 
Set $ d = RK, \lambda = c \sqrt{\log(d)/ d}$.
}
\KwOut{The debiased lasso estimator $\hat{\theta}_d$ and its covariance matrix $\hat{\Sigma}_d $.\\}
Let  $\hat{\theta}_l$ be the lasso estimator calculated by
\eqs{ \label{eq:Lasso}  \hat{\theta}_l  &= \argmin_{\theta} \frac{1}{d} \sum_{r,k} [  n_{rk} e^{x_{rk}^\top\theta } - s_{rk} x_{rk}^\top \theta  ] + \lambda ||\theta||_1     .}

Compute the empirical covariance matrix $ \hat{\Sigma} = \frac{1}{d} \sum_{r,k} n_{rk} e^{x_{rk}^\top \hat{\theta}_l}\cdot x_{rk} x_{rk}^\top.$\\

% \For{$i=1,2, \cdots, d$}{
% $m_i$ is the solution of the convex program:
% \eqs{ \label{eq:smallDebiasCvx}
%  \text{minimize} & ~m^\top \hat{\Sigma} m\\ \nonumber
%  \text{s.t.} & ||\hat{\Sigma} m - e_i||_{\infty } \leq \mu
% }
% where $e_i \in \RR_d$ is the vector with one at the $i$-th position and zero elsewhere.
% }
% Set  $M:= [m_1, \cdots, m_d]^\top$If any of the above problems is not feasible, set $M = I_{d \times d}$.\\. 

Compute the estimator  $\hat{\theta}_d $ and its covariance matrix $  \hat{\Sigma}_d$ as follows:
\eqs{
\hat{\theta}_d &: =  \hat{\theta}_l + \frac{1}{d} \hat{\Sigma}^{-1} \sum_{r,k} (s_{rk} - n_{rk} e^{x_{rk}^\top \hat{\theta}_l}) x_{rk},\text{ and~} \\
\label{eq:dl_cov}
  \hat{\Sigma}_d & = \hat{\Sigma}^{-1} / d. }
\caption{Debiased Lasso Estimator for $\theta$ in High-dimensional Poisson Model}
\label{alg_debiasedLasso}
\end{algorithm}

Conceptually, Algorithm \ref{alg_debiasedLasso}  begins by computing the lasso estimator $\hat{\theta}_l$ from equation \eqref{eq:Lasso}. It then obtains an unbiased estimator $\hat{\theta}_d $ by adding a (small) correction, $\frac{1}{d} \hat{\Sigma}^{-1} \sum_{r,k} (s_{rk} - n_{rk} e^{x_{rk}^\top \hat{\theta}_l}) x_{rk} $, to $\hat{\theta}_l$. The main idea of this debiasing approach is to invert the Karush-Kuhn-Tucker (KKT) characterization of the lasso. Here, unlike in the existing high-dimensional lasso bandit algorithms of \cite{bastani2020online} and \cite{oh2020sparsity}, \comm{we choose the penalty parameter $\lambda = c\sqrt{\log(d)/d}$ according to Theorem 8 in \cite{javanmard2014confidence}
}, which does not shrink as $t$ increases. For a fixed data set, the time for computing \eqref{eq:Lasso}  increases as $\lambda$ decreases, so a constant $\lambda$ implies that the computation time barely changes as $t$ increases, thereby reducing the computation time significantly compared to other methods in which $\lambda$ shrinks over time (see, e.g., Figure \ref{fig:real}). The intuition behind this phenomenon is discussed in Subsection \ref{subsec:pos_features}.

We omit further discussion of this estimator and refer readers to \cite{van2014asymptotically}, \cite{javanmard2014confidence}, and \cite{zhang2014confidence}. Heuristically, the true parameter vector $\theta$ has a distribution similar to $\cN (\hat{\theta}_d, \hat{\Sigma}_d )$. 

\subsection{Generalized Thompson sampling for treatment selection} \label{2sec:treatment}

In the classical Thompson sampling literature \citep{russo2017tutorial}, at each step, the algorithm samples a parameter vector $\tilde{\theta}$ from the current posterior distribution, then selects an action that maximizes the expected reward assuming the true parameter vector equals the sampled value $\tilde{\theta}$. In PMDL, we modify the classical Thompson sampling in two ways. \comm{(HN:This explains what we do, but it will be good to give some intuition for why we do what we do. In particular, why did we choose frequentist Thompson sampling rather than standard Thompson sampling, and what advantage is created by the use of frequentest Thompson sampling?) First, since calculating and sampling from a Bayesian posterior is very complicated in the high-dimensional setting, we instead use the high-probability confidence region computed by the frequentist method. Specifically, we sample $\tilde{\theta}$ from a Gaussian distribution $\cN(\hat{\theta}_d, \alpha\hat{\Sigma}_d )$. Second, to control the rate of exploration, we use an hyper-parameter $\alpha$: when $\alpha = 0,$ PMDL reduces to a greedy method; when $\alpha = 1$, it is the standard form of Thompson Sampling where we directly sample from the ``posterior''. The adjustable exploration idea is also explored in \cite{min2020policy} and \cite{kveton2020randomized}.} How to find the best exploration index is an interesting research problem in its own right, and is beyond the scope of this paper. Instead,  we provide numerical studies in Subsection \ref{subsec:adjustable_exp} on the relationship between the best $\alpha$ and problem dimension $d$.
% Rather than tackling the question of finding the best exploration index (a direction we leave for future work), we instead provide numerical studies in Section \ref{subsec:adjustable_exp}, on the relationship between the best $\alpha$ and problem dimension $d$.

After sampling $\Tilde{\theta}$ from $  \cN(\hat{\theta}_d, \alpha\hat{\Sigma}_d )$, the algorithm computes
\eqss{
\tilde{p}_{rk} & = \exp(\Tilde{\theta}^\top x_{rk}  )}
and sets
\eqss{(r_t, k_t) & = \argmax_{r, k} ~\tilde{p}_{rk}
.}

The various steps that constitute our PMDL method are summarized as Algorithm \ref{alg_PMDL}:
\begin{algorithm}[H]
\KwIn{ $ c, \alpha, \hat{\theta}_d  = [0, 0, \cdots, 0] \in \RR^d, \hat{\Sigma}_d = \vI_d$\\
Set  $d = RK, \lambda = c \sqrt{\log d/ d}$.
}

\For{$t=1,2, \cdots, T$}{
Sample $ \Tilde{\theta} \sim \cN(  \theta_d , \alpha \Sigma_d)$ \\
Select $ (r_t, k_t) = \argmax_{r, k} \sum_{j}  \exp(\Tilde{\theta}^\top x_{rk})  $.\\
Platform sample one user from TA $k_t$ and display CA $r_t$, observe $y_t$.\\
Update $n_{r_t k_t} \leftarrow  n_{r_t k_t}+1, s_{r_t k_t} \leftarrow s_{r_t k_t}+y_t$.\\  
Compute 
 $\hat{\theta}_l  = \argmin_{\theta} \frac{1}{d} \sum_{r,k} [  n_{rk} e^{x_{rk}^\top\theta } - s_{rk} x_{rk}^\top \theta  ] + \lambda ||\theta||_1   $, and $ \hat{\Sigma} = \frac{1}{d} \sum_{r,k} n_{rk} e^{x_{rk}^\top \hat{\theta}_l}\cdot x_{rk} x_{rk}^\top$.\\ 
Update
$\hat{\theta}_d \leftarrow  \hat{\theta}_l + \frac{1}{d} \hat{\Sigma}^{-1} \sum_{r,k} (s_{rk} - n_{rk} e^{x_{r}^\top \hat{\theta}_l}) x_{rk}, \text{ and~}   \hat{\Sigma}_d \leftarrow \hat{\Sigma}^{-1} / d.$ 
}
\caption{PMDL Algorithm}
 \label{alg_PMDL}
\end{algorithm}
\comm{(HN: can we provide the explicit log-likelihood, and  the derivation of the SIGMA term for both the Poisson model and the logistic model in an appendix?)\\

We detail the calculation in the algorithm in Appendix \ref{app:calc}.  }

\subsection{Positive features of PMDL } \label{subsec:pos_features}

We discuss in this section the positive features of the PMDL framework that make it suitable for the high-dimensional online advertising problem. 

\noindent \textbf{Cross-learning}. \quad The combination of high-dimensionality, weak signal (that is, very low CTRs), and short learning horizon ($T$) make it important for the advertiser to be able to use indirect evidence for inference. To understand how PMDL facilitates cross-learning, first consider a two-way additive Poisson regression model $ p_{rk} = e^{c+\alpha_r + \beta_k}$, where all parameters ($c, \alpha_r, \beta_k$) are shared among different arms. Despite its high potential for cross-learning, this model likely suffers from model misspecification; that is, it is likely that no model of this simple form fits the true parameters closely. 

Next, we consider adding interaction terms such that $ p_{rk} = e^{c+\alpha_r + \beta_k + \gamma_{rk}}$. This is referred to as a \textit{hybrid model} in \cite{chapelle2011empirical}, since some of the parameters ($c, \alpha_r, \beta_k$) are shared among all arms, and some are unique to the arm ($\gamma_{rk}$). Introducing interaction terms reduces the potential for model misspecification, but may weaken cross-learning when the model is combined with an unpenalized estimator. For example, denoting by $\Tilde{p}_{rk} = \frac{s_{rk}}{n_{rk}}$ the observed success rate in some number of initial trials, an unpenalized estimation method can achieve a perfect fit to that data by taking $\gamma_{rk} = \log \Tilde{p}_{rk} $ and $c=\alpha_r = \beta_k = 0$ for all $r, k,$ which will have a very poor generalization. The use of the debiased lasso estimator balances the conflicting priorities -- cross-learning versus model misspecification -- by restricting the number of interaction terms (through lasso), which  promotes cross-learning, while constructing an unbiased estimator (through debiasing). 
% We note that this may not be achieved by ridge regression (the estimation method used in LMLA, logit model Laplace approximation, cf. \cite{chapelle2011empirical}) since it does not rule out redundant features but instead tries to make feature parameters small.

\noindent \textbf{Efficient computation}. \quad The computational saving from using a Poisson model instead of logistic model results from the estimation method interacting with the bandit logic. A well-performing bandit algorithm requires that the distance between the estimator and the true parameter, $ ||\hat{\theta} - \theta^*|| $, converges to $0$ as $t$ increases. 

We want to learn how using different regression models may affect the convergence of $ ||\hat{\theta} - \theta^*|| $. When the estimator is generated by a penalized regression,  $ ||\hat{\theta} - \theta^*|| $ is typically bounded by 
\eqs{\label{eq:error} O( \frac{\lambda_t}{\sigma_{\min}(\hat{\Sigma})}),}
where $\lambda_t$ is the penalty rate at time $t$ and $\sigma_{\min}(\hat{\Sigma})$ is the smallest eigenvalue of the empirical covariance matrix, cf. Theorem 6.1 of \cite{buhlmann2011statistics} and \cite{hoerl1970ridge}. The intuition behind \eqref{eq:error} is that an increasing penalty rate $\lambda_t$ encourages the model to be as simple as possible, which increases bias; on the other hand, when there's more variance in the data (that is, $\sigma_{\min}(\hat{\Sigma})$ is larger), the estimation bias decreases. One task in designing a bandit algorithm is to ensure that the error is bounded, as per \eqref{eq:error}. \comm{(HN:Is there any intuition for why the empirical covariance matrix for the poison increases over time while that for the logistic converges to a constant?)}
\begin{itemize}
    \item For our penalized Poisson regression model, which models \textit{counting data} $s_{rk}$ (Algorithm \ref{alg_PMDL}) \comm{with a rate $n_{rk} p_{rk}$ that scales with $n_{rk}$, the empirical covariance matrix has a higher variance as the experiment proceeds. Indeed,} $\hat{\Sigma} = (RK)^{-1} \sum_{r,k} n_{rk} e^{x_{rk}^\top \hat{\theta}_l}\cdot x_{rk} x_{rk}^\top,$ and $\sigma_{\min}(\hat{\Sigma})\uparrow \infty$ as $t \to \infty$. \commm{ Therefore, \eqref{eq:error} is bounded even if we hold the penalty parameter $\lambda$ constant  ($\lambda = c\frac{\log d}{d}$)}.
    
    \item \comm{For a penalized logistic regression that models \textit{trial-by-trial data} (see Algorithm \ref{alg_LMDL} in Subsection \ref{subsec:LMDL}), the empirical covariance matrix converges to a constant matrix as time proceeds. Indeed, $\hat{\Sigma} = \frac{1}{t} \sum_{\tau=1}^t (1+\exp(\hat{\theta}_l^\top x_\tau ))^{-1}(1+\exp(-\hat{\theta}_l^\top x_\tau ))^{-1} x_\tau x_\tau^\top,$ and the denominator in \eqref{eq:error} converges to a constant as $t$ increases. In order to balance that $\lambda$ has to fall.}
\end{itemize}

In summary, a penalized Poisson regression model can use a constant penalty rate, whereas a penalized logistic regression model requires a decaying penalty rate. As commonly observed in the literature (see, e.g., \cite{friedman2008sparse}, Table 2), the computation time of the lasso regression increases drastically as the penalty parameter shrinks. Therefore, a constant penalty in PMDL means that the computation time of lasso at each re-estimation point does not increase much as $t$ increases, whereas the computation time of a penalized logistic regression increases. Indeed, Figure \ref{fig:large_updateTime}(b) in Subsection \ref{subsec:highdimResult} shows the significant computational savings when we switch from a logistic model (SA Lasso) to a Poisson model (PMDL).

The computation savings of the PMDL method relies on the fact that there are only a finite number of CA-TA combinations. When the number of feature vectors is infinite, which is likely to happen when the feature vector involves continuous variables, the PMDL method would have a similar computation time as methods based on the logistic model.


% Poisson regression uses counting data for each CA-TA group instead of individual trial data in the logistic model. As we only have finitely many CA-TA combinations in the model, the number of groups ($RK$) remains the same throughout the experiment. 



%  This is generally achieved by using a smaller penalty parameter $\lambda$ since a smaller $\lambda$ corresponds to a smaller variance in estimators, cf.  $c\sqrt{\log(2dt^2)/t}$ in \cite{li2021simple}, and $\lambda = c \sqrt{(2\log(d) + 4\log(t)/ t}$ in \cite{oh2020sparsity}. In Section \ref{subsec:LMDL}, we describe a method called \textit{Logit Model Debiased Lasso} (LMDL), for general success probability, where we have $\lambda = c \sqrt{\log(d)/ t}.$ Alternatively, if each statistical unit has a higher variance as $t$ grows, it will lower the estimator covariance. Hence, we may not need to reduce the regularization penalty. Indeed, when using penalized Poisson regression, as $t$ grows, there are more samples in each group - despite using a constant penalty rate ($\lambda = c \sqrt{\log(d)/ d}$), PMDL has a shrinking sampling covariance matrix as $t$ grows. 

\noindent \textbf{Adaptability}. \quad For Thompson sampling algorithms, the idea is to first sample a parameter estimate from the posterior distribution (or, as in our setting, from the Gaussian distribution that approximates the distribution of the debiased lasso estimator), and then treat it as the actual parameter for decision-making. Once we have sampled a parameter vector, treatment selection is straightforward. Therefore, Thompson sampling algorithms (hence PMDL) can be easily adjusted to complicated settings, as we will show in Section \ref{sec:twostage}. In contrast, another popular class of bandit algorithms, the upper confidence bound algorithms (UCB), involves calculating an optimistic estimate (upper confidence bound) of the expected reward for each arm. The calculation of the optimistic estimate can be very sensitive to problem complexity, so UCB algorithms are usually applied to problems with a simple structure.
% In Section \ref{sec:twostage}, we present an instance of a complicated scenario where we can easily adjust our sampling-based method to.

